Sublabel-Accurate Discretization of Nonconvex Free-Discontinuity Problems

In this work we show how sublabel-accurate multilabeling approaches can be derived by approximating a classical label-continuous convex relaxation of nonconvex free-discontinuity problems. This insight allows to extend these sublabel-accurate approaches from total variation to general convex and nonconvex regularizations. Furthermore, it leads to a systematic approach to the discretization of continuous convex relaxations. We study the relationship to existing discretizations and to discrete-continuous MRFs. Finally, we apply the proposed approach to obtain a sublabel-accurate and convex solution to the vectorial Mumford-Shah functional and show in several experiments that it leads to more precise solutions using fewer labels.

==> figures/graph_figure/fig_lifting.tex <==
{%\scalefont{0.9}
\begin{tikzpicture}
\begin{axis}[yscale=0.7,axis y line=left, axis x line = bottom,
            xlabel=$\Omega$,
            ylabel=$\Gamma$,
%            enlargelimits,
            xtick={5.5}, %,7,18},
            xticklabels={$p$}, %, $J_u$, $J_u$},
%            axis line style={-Latex[round]},
            axis line style=-,
            ymin=0,
            ymax=21,
            ytick={0,5,10,15,20},
            yticklabels={$\gamma_1$,$\gamma_2$,$\gamma_3$,$\gamma_4$,$\gamma_5$}]
\pgfdeclarelayer{pre main}
\pgfsetlayers{pre main,main}
\addplot[name path=A,gray,domain={0:7},samples=100] {0.7*cos(0.5*x^3-7*x^2+1*x+2)+13-0.09*x};

\addplot[name path=B,gray,domain={7:18},samples=100] {-0.7*cos(0.06*x^3-0.7*x^2+1*x)+3-0.009*x};

\addplot[name path=C,gray,domain={18:30},samples=100] {0.7*cos(0.005*x^3-0.7*x^2+1*x)+10+0.09*x};
\addplot[name path=foo,white,domain={30:32.6},samples=100] {0.7*cos(0.005*x^3-0.7*x^2+1*x)+8+0.09*x};



\draw[color=gray,name path=X] (axis cs:7,{0.7*cos(0.5*7^3-7*7^2+1*10+2)+13-0.09*7}) -- (axis cs:7,{-0.7*cos(0.06*7^3-0.7*7^2+1*7)+3-0.009*7});
%\draw[color=gray,dashed] (axis cs:10,{-0.7*cos(0.06*10^3-0.7*10^2+1*10)+3-0.009*10}) -- (axis cs:10,0);
\draw[color=gray, name path=Y] (axis cs:18,{-0.7*cos(0.06*18^3-0.7*18^2+1*18)+3-0.009*18}) -- (axis cs:18,{0.7*cos(0.005*18^3-0.7*18^2+1*18)+10+0.09*18});
%\draw[color=gray,dashed] (axis cs:20,{-0.7*cos(0.06*20^3-0.7*20^2+1*20)+3-0.009*20}) -- (axis cs:20,0);

\node[fill=black,circle,inner sep=0pt,minimum size=4pt] at (axis cs: 5.5,{0.7*cos(0.5*5.5^3-7*5.5^2+1*5.5)+13-0.09*5.5}){};
%\node[black,above] at (axis cs:13.3,{0.7*cos(0.5*5.5^3-7*5.5^2+1*5.5)+13-0.09*5.5+0.2}){$\begin{aligned}&\sum e_i\int_{\Gamma} \Phi^0_i(t) \mathbf{1}_u(p, t) \mathrm{d}t =\\ &~h \cdot \begin{bmatrix} 1 & 1 & 0.4 & 0\end{bmatrix}^\top\end{aligned}$};

\node at (axis cs:12.5, 5.5){$\mathbf{1}_u \equiv 0$};
\node at (axis cs:24.5, 5.5){$\mathbf{1}_u \equiv 1$};
\node at (axis cs:31.5, 12.6){$G_u$};
\node at (axis cs:19.4, 3.8){$u^-$};
\node at (axis cs:18.5, 12.1){$u^+$};

\draw[color=black!50!white,dashed] (axis cs:7,0) -- (axis cs:7,{0.7*cos(0.5*7^3-7*7^2+1*7)+13-0.09*7});
\draw[color=black!50!white,dashed] (axis cs:18,0) -- (axis cs:18,{-0.7*cos(0.06*18^3-0.7*18^2+1*18)+3-0.009*18});
\draw[color=black!50!white,dashed] (axis cs:5.5,0) -- (axis cs:5.5,{0.7*cos(0.5*5.5^3-7*5.5^2+1*5.5)+13-0.09*5.5});
\draw[color=black!50!white,dashed] (axis cs:0,{0.7*cos(0.5*5.5^3-7*5.5^2+1*5.5)+13-0.09*5.5}) -- (axis cs:5.5,{0.7*cos(0.5*5.5^3-7*5.5^2+1*5.5)+13-0.09*5.5});

\draw[arrows=->,>=stealth,line width=.5pt](18,9)--(19.1,9);
\draw[arrows=->,>=stealth,line width=.5pt](20,11.25)--(20.2,10);
\node at (axis cs:20.7, 9){$\nu_{G_u}$};

\path[name path=axis] (axis cs:0,0) -- (axis cs:30,0);

\addplot [
        thick,
        color=gray,
        fill=gray,  
        fill opacity=0.15
    ]
    fill between[
        of=A and axis,
        soft clip={domain=0:7},
    ];
\addplot [
        thick,
        color=gray,
        fill=gray,  
        fill opacity=0.15
    ]
    fill between[
        of=B and axis,
        soft clip={domain=7:18},
    ];
\addplot [
        thick,
        color=gray,
        fill=gray, 
        fill opacity=0.15
    ]
    fill between[
        of=C and axis,
        soft clip={domain=18:31},
    ];
    
\end{axis}
\end{tikzpicture}}


